A Genetic Algorithm-based Framework for Learning Statistical Power Manifold

Statistical power is a measure of the replicability of a categorical hypothesis test. Formally, it is the probability of detecting an effect, if there is a true effect present in the population. Hence, optimizing statistical power as a function of some parameters of a hypothesis test is desirable. However, for most hypothesis tests, the explicit functional form of statistical power for individual model parameters is unknown; but calculating power for a given set of values of those parameters is possible using simulated experiments. These simulated experiments are usually computationally expensive. Hence, developing the entire statistical power manifold using simulations can be very time-consuming. We propose a novel genetic algorithm-based framework for learning statistical power manifolds. For a multiple linear regression $F$-test, we show that the proposed algorithm/framework learns the statistical power manifold much faster as compared to a brute-force approach as the number of queries to the power oracle is significantly reduced. We also show that the quality of learning the manifold improves as the number of iterations increases for the genetic algorithm. Such tools are useful for evaluating statistical power trade-offs when researchers have little information regarding a priori best guesses of primary effect sizes of interest or how sampling variability in non-primary effects impacts power for primary ones.

==> sections/abstract.tex <==
\begin{abstract}
Statistical power is a measure of the goodness/strength of a hypothesis test. Formally, it is the probability of detecting an effect, if there is a true effect present to detect. Hence, optimizing statistical power as a function of some parameters of a hypothesis test is desirable. However, for most hypothesis tests, the explicit functional form of statistical power as a function of those parameters is unknown but calculating statistical power for a given set of values of those parameters is possible using simulated experiments. These simulated experiments are usually computationally expensive. Hence, developing the entire statistical power manifold using simulations can be very time-consuming. Motivated by this, we propose a novel genetic algorithm-based framework for learning statistical power manifold. For a multiple linear regression $F$-test, we show that the proposed algorithm/framework learns the statistical power manifold much faster as compared to a brute-force approach as the number of queries to the power oracle is significantly reduced. We also show that the quality of learning the manifold improves as the number of iterations increases for the genetic algorithm.
\end{abstract}

==> sections/abstract_ieee.tex <==
\begin{abstract}
Statistical power is a measure of the goodness/strength of a hypothesis test. Formally, it is the probability of detecting an effect, if there is a true effect present to detect. Hence, optimizing statistical power as a function of some parameters of a hypothesis test is desirable. However, for most hypothesis tests, the explicit functional form of statistical power as a function of those parameters is unknown but calculating statistical power for a given set of values of those parameters is possible using simulated experiments. These simulated experiments are usually computationally expensive. Hence, developing the entire statistical power manifold using simulations can be very time-consuming. Motivated by this, we propose a novel genetic algorithm-based framework for learning statistical power manifold. For a multiple linear regression $F$-test, we show that the proposed algorithm/framework learns the statistical power manifold much faster as compared to a brute-force approach as the number of queries to the power oracle is significantly reduced. We also show that the quality of learning the manifold improves as the number of iterations increases for the genetic algorithm.
\end{abstract}

\begin{IEEEkeywords}
Statistical power, hypothesis testing, genetic algorithm, nearest neighbors
\end{IEEEkeywords}

==> sections/data_and_code.tex <==
\paragraph*{Data and Code Availability}
This research involves simulations but no real data. The source code for our experiments is available \href{https://drive.google.com/drive/folders/1xO3S_r-XfF4nPPN1aB30ByKzRnsdojjx?usp=sharing}{here}. 

%This initial paragraph is \textbf{mandatory}. Briefly state what data you use (including citations if appropriate) and whether the data are available to other researchers.\footnote{An example data availability statement: This paper uses the MIMIC-III dataset \citep{johnson2016mimic}, which is available on the PhysioNet repository \citep{johnson2016physionet}.} If you are not sharing code, you must explicitly state that you are not making your code available. If you are making your code available, then at the time of submission for review, please include your code as supplemental material or as a code repository link; in either case, your code must be anonymized. If your paper is accepted, then you should de-anonymize your code for the camera-ready version of the paper. \emph{If you do not include this data and code availability statement for your paper, or you provide code that is not anonymized at the time of submission, then your paper will be desk-rejected.} Your experiments later could refer to this initial data and code availability statement if it is helpful (e.g., to avoid restating what data you use).

==> sections/irb.tex <==
\section*{Institutional Review Board (IRB)}
This research doesn't require IRB approval.
%This section is \textbf{mandatory}. If your research requires IRB approval or has been designated by your IRB as Not Human Subject Research, then for the camera-ready version of the paper, you must provide IRB information (and at the time of submission for review, you can say that this IRB information will be provided if the paper is accepted). If your research does not require IRB approval, then you must state this to be the case. This section does not count toward the paper page limit.

==> sections/plots_beta1.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_1000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_1000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_1000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_1000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_1$ and $n$ vs. no. of iterations when population size is 1000.} \label{fig:qualityoflearning11000}
\end{figure*}

\if 0
\begin{figure*}[t]
\centering
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_2000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_2000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_2000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_2000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_1$ and $n$ vs. no. of iterations when population size is 2000.} \label{fig:qualityoflearning12000}
\end{figure*}
\fi

\begin{figure*}[t]
\centering
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_3000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_3000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_3000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_3000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_1$ and $n$ vs. no. of iterations when population size is 3000.} \label{fig:qualityoflearning13000}
\end{figure*}

\if 0
\begin{figure*}[t]
\centering
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_4000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_4000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_4000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_4000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_1$ and $n$ vs. no. of iterations when population size is 4000.} \label{fig:qualityoflearning14000}
\end{figure*}
\fi

\begin{figure*}[t]
\centering
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_5000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.20\textwidth}
  \centering
  \subcaption{\#(iterations) = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_5000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_5000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{\#(iterations) = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_5000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.19\textwidth}
  \centering
  \subcaption{brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta1_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_1$ and $n$ vs. no. of iterations when population size is 5000.} \label{fig:qualityoflearning15000}
\end{figure*}

==> sections/plots_beta3_old.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_1000_10.jpg}}
  \subcaption{$I$ = 10}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_1000_20.jpg}}
  \subcaption{$I$ = 20}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_1000_50.jpg}}
  \subcaption{$I$ = 50}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_1000_70.jpg}}
  \subcaption{$I$ = 70}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_1000_100.jpg}}
  \subcaption{$I$ = 100}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_bf.jpg}}
  \subcaption{Brute-force}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_3$ and $n$ vs. no. of iterations when population size is 1000.} \label{fig:qualityoflearning31000}
\end{figure*}

\begin{figure*}[t]
\centering
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_10.jpg}}
  \subcaption{$I$ = 10}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_20.jpg}}
  \subcaption{$I$ = 20}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_50.jpg}}
  \subcaption{$I$ = 50}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_70.jpg}}
  \subcaption{$I$ = 70}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_100.jpg}}
  \subcaption{$I$ = 100}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_bf.jpg}}
  \subcaption{Brute-force}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_3$ and $n$ vs. no. of iterations when population size is 2000.} \label{fig:qualityoflearning32000}
\end{figure*}

\begin{figure*}[t]
\centering
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_2000_70.jpg}}
  \subcaption{$I$ = 10}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_3000_20.jpg}}
  \subcaption{$I$ = 20}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_3000_50.jpg}}
  \subcaption{$I$ = 50}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_3000_70.jpg}}
  \subcaption{$I$ = 70}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_3000_100.jpg}}
  \subcaption{$I$ = 100}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_bf.jpg}}
  \subcaption{Brute-force}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_3$ and $n$ vs. no. of iterations when population size is 3000.} \label{fig:qualityoflearning33000}
\end{figure*}

\if 0
\begin{figure*}[t]
\centering
\begin{minipage}{.33\textwidth}
  \centering
  \subcaption{$I$ = 10}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_4000_10.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.33\textwidth}
  \centering
  \subcaption{$I$ = 20}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_4000_20.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.33\textwidth}
  \centering
  \subcaption{$I$ = 50}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_4000_50.jpg}}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.33\textwidth}
  \centering
  \subcaption{$I$ = 70}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_4000_70.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.33\textwidth}
  \centering
  \subcaption{Brute-force}
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_bf.jpg}}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_3$ and $n$ vs. no. of iterations when population size is 4000.} \label{fig:qualityoflearning34000}
\end{figure*}
\fi

\begin{figure*}[t]
\centering
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_5000_10.jpg}}
  \subcaption{$I$ = 10}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_5000_20.jpg}}
  \subcaption{$I$ = 20}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_5000_50.jpg}}
  \subcaption{$I$ = 50}
  %\label{fig:facebook-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_5000_70.jpg}}
  \subcaption{$I$ = 70}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_5000_100.jpg}}
  \subcaption{$I$ = 100}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics{figures/power_vs_beta3_and_sample_size_bf.jpg}}
  \subcaption{Brute-force}
  %\label{fig:bitcoin-lt-wc}
\end{minipage}
\caption{Quality of learning the power manifold as a function of $\beta_3$ and $n$ vs. no. of iterations when population size is 5000.} \label{fig:qualityoflearning35000}
\end{figure*}
